BanditWare: A Contextual Bandit-based Framework for Hardware Prediction

Distributed computing systems are essential for meeting the demands of modern applications, yet transitioning from single-system to distributed environments presents significant challenges. Misallocating resources in shared systems can lead to resource contention, system instability, degraded performance, priority inversion, inefficient utilization, increased latency, and environmental impact. We present BanditWare, an online recommendation system that dynamically selects the most suitable hardware for applications using a contextual multi-armed bandit algorithm. BanditWare balances exploration and exploitation, gradually refining its hardware recommendations based on observed application performance while continuing to explore potentially better options. Unlike traditional statistical and machine learning approaches that rely heavily on large historical datasets, BanditWare operates online, learning and adapting in real-time as new workloads arrive. We evaluated BanditWare on three workflow applications: Cycles (an agricultural science scientific workflow) BurnPro3D (a web-based platform for fire science) and a matrix multiplication application. Designed for seamless integration with the National Data Platform (NDP), BanditWare enables users of all experience levels to optimize resource allocation efficiently.

==> sec-pt2_experiments.tex <==
\section{Experiments Part 2: Matrix Multiplication}
\subsection{Use-Case}
We demonstrate the effectiveness of BanditWare with a more hardware-sensitive application: A simple parallelized matrix multiplication. Specifically, a tiled, parallelized matrix squaring program run on a square matrix. Each core is assigned a set of unique tiles to calculate in the final matrix, splitting up the work among all available cores. Since this program uses multiprocessing, different hardware configurations had a more prominent effect on the runtime of the application, contrasting the results from BP3D.


\subsection{Matrix Squaring}
We chose a matrix squaring algorithm rather than matrix multiplication between two different matrices to reduce the number of parameters, allowing for a more focused analysis. In order to generate the matrices to be squared, a separate program was used to create the matrix given certain parameters. This program takes in the sparsity (ratio of 0s in the matrix to total cells) and size of the matrix, as well as the minimum and maximize permitted values, returning a matrix of randomized integers with those specifications. This generation time was not counted in the recorded runtime, but these matrix generation input parameters were recorded to give information about the matrices for better runtime prediction. We keep the generation time separate from the matrix squaring time because we are only analyzing the matrix squaring application.

For our Matrix Squaring dataset, we ran the application on a large variety of inputs, creating a quite varied outputs. We enumerated the runs over a set of values for size, sparsity, min, and max to create a dataset with a total of 2,520 runs. In just the \texttt{size} parameter, we have inputs ranging from 100 to 12,500, resulting in outputs with a minimum runtime of 0 seconds and a maximum runtime of 1,797 seconds (nearly half an hour).

To show the strengths and limitations of our model, we ran it on the entire dataset as well as a limited portion of the dataset that only contained inputs from size 5,000 to 12,500, with a total of 720 data points. By limiting it to these larger sizes, we should expect a hardware with many CPU cores to thrive, as opposed to the entire dataset, where the large proportion of low sizes would encourage a hardware with fewer cores, meaning less multiprocessing overhead. 
%As mentioned earlier, with a dataset of runs that has highly variable hardware needs, the accuracy is bound to suffer due to the constraint that we must choose one hardware that best fits the entire dataset. Thus, we should expect to see a somewhat low accuracy on the entire dataset but a higher accuracy on the truncated dataset.


\subsection{Matrix Squaring Results (Linear Regression)}
To achieve a baseline of predictive results, we employ a simple linear regression approach to recommend hardware configurations using the Matrix Squaring dataset.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{figs/matmul_rmse.png}
        \caption{RMSE scores}
    \end{subfigure}%
    
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{figs/matmul_duration.png}
        \caption{Duration (seconds)}
    \end{subfigure}
    \caption{RMSE scores and training duration (s) of 100 linear regression recommendation models trained on matrix squaring data.}
    \label{fig:lr_recommender}
\end{figure}



\subsection{Matrix Squaring Results}
Running BanditWare on the entire dataset, we can see that the accuracy is relatively low. 


